Parameterized Complexity and Approximability of Directed Odd Cycle Transversal

A directed odd cycle transversal of a directed graph (digraph) $D$ is a vertex set $S$ that intersects every odd directed cycle of $D$. In the Directed Odd Cycle Transversal (DOCT) problem, the input consists of a digraph $D$ and an integer $k$. The objective is to determine whether there exists a directed odd cycle transversal of $D$ of size at most $k$. In this paper, we settle the parameterized complexity of DOCT when parameterized by the solution size $k$ by showing that DOCT does not admit an algorithm with running time $f(k)n^{O(1)}$ unless FPT = W[1]. On the positive side, we give a factor $2$ fixed parameter tractable (FPT) approximation algorithm for the problem. More precisely, our algorithm takes as input $D$ and $k$, runs in time $2^{O(k^2)}n^{O(1)}$, and either concludes that $D$ does not have a directed odd cycle transversal of size at most $k$, or produces a solution of size at most $2k$. Finally, we provide evidence that there exists $\epsilon > 0$ such that DOCT does not admit a factor $(1+\epsilon)$ FPT-approximation algorithm.

==> doct_preamble.tex <==
\newcommand{\longversion}[1]{{#1}
\newcommand{\shortversion}[1]}

\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{soul}
\newcommand{\hlr}[1]{\sethlcolor{Salmon1}\hl{#1}\sethlcolor{yellow}} 
\newcommand{\hlg}[1]{\sethlcolor{PaleGreen2}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlb}[1]{\sethlcolor{SkyBlue1}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlo}[1]{\sethlcolor{Apricot}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hly}[1]{\sethlcolor{Gold}\hl{#1}\sethlcolor{yellow}}
\usepackage{listings}
\usepackage{mathrsfs}
\usepackage[mathscr]{euscript}
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amstext}
\usepackage{graphicx,tikz}
\RequirePackage{fancyhdr}
\usepackage{xcolor}
\usepackage{boxedminipage}
\usepackage[linesnumbered, boxed, algosection,noline]{algorithm2e}
\usepackage{graphics}
\usepackage{pgf}
\usepackage{paralist} 
\usepackage{framed}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{enumerate}
\usepackage{float}
\usepackage{xspace}
\usepackage{todonotes}



\newcommand{\cR}{\mathcal{R}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\doctfunc}[1]{{\sf doct}{(#1)}}

\usepackage{vmargin}
\setmarginsrb{1in}{1in}{1in}{1in}{0pt}{0pt}{0pt}{6mm}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1}}}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}[section]
\newtheorem{claim}{Claim}[section]
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{redrule}{Reduction Rule}[section]
\newtheorem{remark}{Remark}
\newtheorem{reduction}{Reduction Rule}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{hypothesis}{Hypothesis}

\date{}
 
\newcommand{\defparproblem}[4]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
}\vspace{1mm}}

\newcommand{\defproblem}[3]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #3
  \end{minipage}
}\vspace{1mm}}

\newcommand{\parnamedefn}[4]{
\begin{tabbing}
\name{#1} \\
\emph{Input:} \hspace{1cm} \= \parbox[t]{10cm}{#2} \\
\emph{Parameter:}            \> \parbox[t]{10cm}{#3} \\
\emph{Question:}             \> \parbox[t]{10cm}{#4} \\
\end{tabbing}
\vspace{-0.5cm}}

\newcommand{\decnamedefn}[3]{
\begin{tabbing} #1\\
\emph{Input:} \hspace{1.2cm} \= \parbox[t]{12cm}{#2} \\
\emph{Question:}             \> \parbox[t]{12cm}{#3}
\end{tabbing}}

\newcommand{\csplong}{{\sc Binary Constraint Satisfaction Problem}}
\newcommand{\cspshort}{{\sc BCSP}}
\newcommand{\cspt}{{\sc BCSP$_3$}}
\newcommand{\pre}{\mathrm{pre}\xspace}
\newcommand{\post}{\mathrm{post}\xspace}
\newcommand{\bigoh}{{\mathcal{O}}}
\newcommand{\yes}{{yes}}
\newcommand{\no}{{no}}
\newcommand{\yesinstance}{\yes-instance\xspace}
\newcommand{\noinstance}{\no-instance\xspace}
\newcommand{\tw}{\textsc{tw}\xspace}
\newcommand{\torso}{\text{\bf torso}\xspace}
\newcommand{\NP}{\text{\normalfont  NP}}
\newcommand{\coNP}{\text{\normalfont co-NP}}
\newcommand{\ETH}{\textsf{ETH}\xspace}
\newcommand{\PIH}{\textsf{PIH}\xspace}
\newcommand{\FPT}{\textsf{FPT}\xspace}
\newcommand{\XP}{\text{\normalfont XP}}
\newcommand{\W}[1][xxxx]{\text{\normalfont W[#1]}\xspace}
\newcommand{\tausat}{\tau_{\textup{SAT}}}
\newcommand{\poly}{\text{\normalfont  poly}}
\newcommand{\ie}{i.e.\xspace}
\newcommand{\WO}{\textsf{W[1]}}
\newcommand{\WOH}{\textsf{W[1]}-hard}
\newcommand{\WOC}{\textsf{W[1]}-complete}
\newcommand{\WTH}{\textsf{W[2]}-hard}
\newcommand{\WTC}{\textsf{W[2]}-complete}
\newcommand{\NPH}{\textsf{NP}-hard}
\newcommand{\NPC}{\textsf{NP}-complete}
\newcommand{\dfvs}{{\sc DFVS}}
\newcommand{\dfas}{{\sc DFAS}}
\newcommand{\sfvs}{{\sc Subset FVS}}
\newcommand{\fvs}{{\sc Feedback Vertex Set}}
\newcommand{\delqbackdoor}{{\sc Deletion \qhorn\ Backdoor Set Detection}}
\newcommand{\optdelqbackdoor}{{\sc Deletion \qhorn\ Backdoor Set Detection}}
\newcommand{\strongqbackdoor}{{\sc Strong} $q$-{\sc Horn Backdoor Set Detection}}
\newcommand{\skewsymmc}{$d$-{\sc Skew-Symmetric Multicut}}
\newcommand{\oneskewsymmc}{$1$-{\sc Skew-Symmetric Multicut}}
\newcommand{\threeskewsymmc}{$3$-{\sc Skew-Symmetric Multicut}}
\newcommand{\edgebip}{{\sc Edge Bipartization}}
\newcommand{\qhorn}{\text{\normalfont{$q$-Horn}}}
\newcommand{\horn}{\text{\normalfont{Horn}}}
\newcommand{\rhorn}{\text{\normalfont{RHorn}}}
\newcommand{\twocnf}{2-\text{\normalfont{CNF}}}
\newcommand{\qhbd}{$\qhorn$-{\sc Backdoor Deletion}}
\newcommand{\almostqhorn}{{\sc Almost} $\qhorn$}
\newcommand{\almostqhorntwo}{{\sc Almost} $\qhorn$}
\newcommand{\almsat}{{\sc Almost} $2$-{\sc SAT}$(v)$}
\newcommand{\almsatc}{{\sc Almost} $2$-{\sc SAT}}
\newcommand{\agvcfull}{{\sc Above Guarantee Vertex Cover}}
\newcommand{\agvc}{{\sc AGVC}}
\newcommand{\mwc}{{\sc  Multiway Cut}}
\newcommand{\emwcfull}{{\sc  Edge Multiway Cut}}
\newcommand{\emwc}{{\sc  EMWC}}
\newcommand{\dfvsfull}{{\sc Directed Feedback Vertex Set}}
\newcommand{\KE}{K\"{o}nig-Egerv\'{a}ry}
\newcommand{\opt}{{\sc OPT}}
\newcommand{\omwcfull}{{\sc Odd Multiway Cut}}
\newcommand{\soct}{{\sc Subset OCT}}
\newcommand{\oct}{{\sc OCT}}
\newcommand{\doctfull}{{\sc Directed Odd Cycle Transversal}\xspace}
\newcommand{\doct}{{\sc DOCT}\xspace}
\newcommand{\flowred}{{\sc Flow Reduction}}
\newcommand{\soctco}{{\sc Subset OCT Compression}}
\newcommand{\soctcstar}{{\sc Subset OCT Compression*}}
\newcommand{\soctc}{{\sc Subset OCT Compression*}}
\newcommand{\omwc}{{\sc OMWC}}
\newcommand{\oemwcfull}{{\sc Odd Edge Multiway Cut}}
\newcommand{\oemwc}{{\sc OEMWC}}
\newcommand{\octfull}{{\sc Odd Cycle Transversal}}
\newcommand{\No}{{\sc No}}
\newcommand{\Yes}{{\sc Yes}}
\newcommand{\Oh}{{\mathcal{O}}}
\newcommand{\set}[2]{\ensuremath{{\cal {#1}}(#2)}}
\newcommand{\setp}[2]{\ensuremath{{\cal {#1}}(S_{#2})}}
\newcommand{\setn}[2]{\ensuremath{{\cal {#1}}(S_{\bar{#2}})}}
\newcommand{\SB}{\{\,}
\newcommand{\SM}{\;{:}\;}
\newcommand{\SE}{\,\}}
\newcommand{\Card}[1]{|#1|}
\newcommand{\CCard}[1]{\|#1\|}
\newcommand{\D}[1]{\mbox{D$($#1$)$}}
\newcommand{\var}{\mbox{var}}
\newcommand{\lit}{\mbox{lit}}
\newcommand{\true}{\mbox{true}}
\newcommand{\false}{\mbox{false}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\tail}{\mbox{\bf Tail}}
\newcommand{\head}{\mbox{\bf Head}}
\newcommand{\pp}[1]{\ensuremath{#1_+}} 
\newcommand{\nn}[1]{\ensuremath{#1_-}} 
\newcommand{\pn}[1]{\ensuremath{#1_{\pm}}} 
\newcommand{\twosat}{\ensuremath{2}-SAT} 
\newcommand{\hy}{\hbox{-}\nobreak\hskip0pt}
\newcommand{\justminus}{-}
\newcommand{\name}[1]{\textsc{#1}}

\usepackage{booktabs}
\usepackage[pdftex, plainpages = false, pdfpagelabels, 
                 %pdfpagelayout = useoutlines,
                 bookmarks=false,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = true,  % was true
                 linkcolor = blue,
                 urlcolor  = blue,
                 citecolor = red,
                 anchorcolor = green,
                 hyperindex = true,
                 hyperfigures
                 ]{hyperref} 


